Quantum Algorithms for Simulating the Lattice Schwinger Model

The Schwinger model (quantum electrodynamics in 1+1 dimensions) is a testbed for the study of quantum gauge field theories. We give scalable, explicit digital quantum algorithms to simulate the lattice Schwinger model in both NISQ and fault-tolerant settings. In particular, we perform a tight analysis of low-order Trotter formula simulations of the Schwinger model, using recently derived commutator bounds, and give upper bounds on the resources needed for simulations in both scenarios. In lattice units, we find a Schwinger model on $N/2$ physical sites with coupling constant $x^{-1/2}$ and electric field cutoff $x^{-1/2}\Lambda$ can be simulated on a quantum computer for time $2xT$ using a number of $T$-gates or CNOTs in $\widetilde{O}( N^{3/2} T^{3/2} \sqrt{x} \Lambda )$ for fixed operator error. This scaling with the truncation $\Lambda$ is better than that expected from algorithms such as qubitization or QDRIFT. Furthermore, we give scalable measurement schemes and algorithms to estimate observables which we cost in both the NISQ and fault-tolerant settings by assuming a simple target observable---the mean pair density. Finally, we bound the root-mean-square error in estimating this observable via simulation as a function of the diamond distance between the ideal and actual CNOT channels. This work provides a rigorous analysis of simulating the Schwinger model, while also providing benchmarks against which subsequent simulation algorithms can be tested.

==> qubitizationStuff.tex <==

\section{Review of Qubitization and Quantum Signal Processing}
Qubitization and quantum signal processing are two techniques that have recently taken the quantum simulation community by storm.
The idea of qubitization has actually been known for quite some time.
It is based on earlier work by Andrew Childs, which showed that for every continuous time evolution there exists an equivalent quantum walk.  Specifically, for any $H\in \mathbb{C}^{2^n \times 2^n}=\sum_{j} h_j U_j$ where the $U_j$ are  unitary matrices and $h_j \ge 0$, a walk operator $W\in \mathbb{C}^{2\times 2} \otimes \mathbb{C}^{2^n \times 2^n}$ can be constructed such that
\begin{equation}
    W = e^{-i \cos^{-1} \left(\frac{\sigma_y \otimes H}{\|H\|_{l_1}}\right)}.
\end{equation}
Here $\|H\|_{l_1} = \sum_j h_j \ge \|H\|$ is a normalizing factor.  Note that this evolution necessitates introducing an additional qubit, which earns it the name qubitization.

Earlier work corrected the spectrum of this operator through the use of phase estimation.  However, later Guang-Hao Low and Isaac Chuang proposed using a technique called quantum signal processing to efficiently transform the spectrum of $W$ to undo the $\cos^{-1}(\cdot)$ in $W$ and recover true Hamiltonian evolution through the introduction of controlled rotation gates that are cunningly interspersed throughout the evolution.  This process replaces the $O(1/\epsilon)$ overheads from older walk-based approaches with an additive $O(\log(1/\epsilon))$ overhead.

In this section, we provide more detail on how this construction works and in particular discuss the methods for inputting the details of the Hamiltonian (specifically the $h_j$ and the $U_j$) into the simulator.  This discussion is essential because without it our discussion needs to be focused only on query complexity, which makes it difficult to compare the costs of qubitization to other simulation methods that use different access models for the Hamiltonian matrix (such as Trotter-Suzuki decompositions for example).

The two main subroutines that are used to bring data into the simulation are commonly referred to as \texttt{SELECT} and \texttt{PREPARE} in the literature~\cite{}.  These subroutines are not only ubiquitous in qubitization, but also in linear combinations of unitaries methods~\cite{}.  The purpose of the \select, is to select a unitary matrix when queried.  In particular,
\begin{equation}
    \select = \sum_j \ket{j}\!\bra{j} \otimes U_j,
\end{equation}
where recall that $H= \sum_j h_j U_j$ for unitary matrices $U_j$.  The \prepare oracle, on the other hand, takes the form
\begin{equation}
    \prepare \ket{0} = \sum_{j} \sqrt{\frac{h_j}{\|H\|_{l_1}}} \ket{j}.
\end{equation}
Note that we only need to define the action of unitary operation \prepare on the $\ket{0}$ state, and a detailed analysis of the qubitization algorithm reveals that its action on the orthogonal compliment is irrelevant.

\section{Implementing Select and Prepare Circuits}

The representation of the diagonal $E_r^2$  term presents the greatest challenge in our circuit design.  Since Pauli-operators form a complete operator basis, it is always possible in principle to find a Pauli-decomposition of $I\otimes E_r^2$ for any $n$.  The cost of this decomposition is exponential, however, so we use a decomposition of the term into a sum of signature matrices following~\cite{}.

The idea behind a decomposition into a sum of signature matrices is simple.  We wish to express $E_r^2 = \sum_{j=1}^{K^2} S_j$ where
\begin{equation}
 \bra{x} S_j \ket{y} = \delta_{x,y} \begin{cases}1 & j \le x^2 \\ (-1)^j& \text{otherwise} \end{cases}
\end{equation}
For example,
\begin{align}
    \begin{bmatrix}4 & 0 & 0 &0 &0 \\ 0&1 &0 &0&0 \\ 0&0&0&0&0 \\ 0&0&0&1&0\\0&0&0&0&4 \end{bmatrix}&\approx  \begin{bmatrix}1 & 0 & 0 &0 &0 \\ 0&1 &0 &0&0 \\ 0&0&1&0&0 \\ 0&0&0&1&0\\0&0&0&0&1 \end{bmatrix} + \begin{bmatrix}1 & 0 & 0 &0 &0 \\ 0&1 &0 &0&0 \\ 0&0&-1&0&0 \\ 0&0&0&1&0\\0&0&0&0&1 \end{bmatrix} + \begin{bmatrix}1 & 0 & 0 &0 &0 \\ 0&1 &0 &0&0 \\ 0&0&1&0&0 \\ 0&0&0&1&0\\0&0&0&0&1 \end{bmatrix}\nonumber\\
    &\qquad+\begin{bmatrix}1 & 0 & 0 &0 &0 \\ 0&-1 &0 &0&0 \\ 0&0&-1&0&0 \\ 0&0&0&-1&0\\0&0&0&0&1 \end{bmatrix}=\begin{bmatrix}4 & 0 & 0 &0 &0 \\ 0&2 &0 &0&0 \\ 0&0&0&0&0 \\ 0&0&0&2&0\\0&0&0&0&4 \end{bmatrix}
\end{align}
Note that this decomposition, which is of the form $H\approx \sum_{j=1}^4 S_j$, errs only in every odd indexed diagonal entry (starting from $0$).

%In the following let us assume that $K$ is even.  Since the cutoff has no physical significance outside of the simulation, we can always choose $K$ to be even.  
Let us consider how to correct this deviation.
Since we anticipate spanning the Hilbert space using qubits, we will have even dimensionality, and therefore asymmetric E-field bounds;
for definiteness, let us take 
\begin{equation}
    -K \leq E_r \leq K-1 \ .
\end{equation}
With this convention, the cutoff $K$ is synonymous with the max E-field value, and $K$ is necessarily even provided the number of qubits is at least two.
Now, because the largest entry of $E_r^2$ is even, it is straight forward to see that every odd-valued in the naive signature sum will be erroneous.  We can correct this by subtly changing the decomposition:
\begin{equation}
 \bra{x} S_{K^2+p} \ket{y} = \delta_{x,y} \left((-1)^{p(x+1{~\rm mod~}2)} \right).
\end{equation}
Thus we have that
\begin{equation}
H =  \sum_{j=1}^{K^2} S_j + \frac{1}{2}\left(S_{K^2+1} +S_{K^2 +2}\right). 
\end{equation}
Each of these  $S_j$ are clearly unitary and so the resultant expansion is a linear combination of unitary matrices, as required for the select oracle used within qubitization.

$\bullet$ Action of the $j^{\text{th}}$ unitary on some basis ket $\ket{i}$: (come up with definition or more clear squaring circuit)
\begin{equation*}
\Qcircuit  {
\lstick{\ket{i} }& {/^n}\qw & \multigate{1}{(\cdot)^2} &  \qw &  \qw & \qw & \multigate{1}{\left[(\cdot)^2\right]^{-1}} & \qw & \rstick{\ket{i}(-)^{S_j(i)}}\\
\lstick{\ket{0}^{\otimes 2n}}  & {/^{2n}}\qw & \ghost{(\cdot)^2} & \multigate{2}{\text{CMP}} & \qw & \multigate{2}{\text{CMP}^{-1}}  & \ghost{ \left[(\cdot)^2\right]^{-1} }  & \qw & \rstick{\ket{0}^{\otimes 2n}}\\
\lstick{\ket{j}} & {/^{2n}}\qw & \qw & \ghost{\text{CMP}} & \gate{1^{\otimes (2n-1)} \otimes Z } & \ghost{\text{CMP}^{-1}} & \qw & \qw & \rstick{\ket{j}}\\
\lstick{\ket{0}} & \qw & \qw & \ghost{\text{CMP}} & \ctrl{-1} & \ghost{\text{CMP}^{-1}} & \qw & \qw & \rstick{\ket{0}}
}
\end{equation*}
$\bullet$ Comparison gate (basically a subtractor):
\begin{equation*}
\Qcircuit  {
\lstick{\ket{i} }& {/^{2n}}\qw & \multigate{2}{\text{CMP}} &  {\hspace{-.8cm}/}\qw &  \rstick{\ket{i}}\\
\lstick{\ket{j}}  & {/^{2n}}\qw & \ghost{\text{CMP}} & {\hspace{-.8cm}/}\qw & \rstick{\ket{j}}\\
\lstick{\ket{0}} & \qw & \ghost{\text{CMP}} & \qw & \rstick{\ket{i>j?}} 
}
\end{equation*}


\textbf{Binary Decomposition.}
We wish to decompose operators $E_r^2$ as a sum of unitaries. Let us assume that the electric field cutoff is given by an integer $K$ then $E_r^2={\rm diag}(K^2,K^2-1,\cdots,0,\cdots,K^2-1,K^2)$. Each integer on the diagonal we can represent using its binary representation, e.g. $K^2=\sum\limits_{i=0}^{\ceil{\log{ K^2}}}b_i 2^i$, where $b_i = 0,1$ are corresponding bit values. Rescaling $b_i$'s to take on values $-1,1$ we can write $E_r^2$ as a sum of $-1,1$ diagonal matrices of the at most depth $\ceil{\log{ K^2}}+1$ i.e. it is logarithmic in the cutoff square. For example,
\begin{align}
    \begin{bmatrix}4 & 0 & 0 &0 &0 \\ 0&1 &0 &0&0 \\ 0&0&0&0&0 \\ 0&0&0&1&0\\0&0&0&0&4 \end{bmatrix}& =  2^{0}\begin{bmatrix}0 & 0 & 0 &0 &0 \\ 0& 1 &0 &0&0 \\ 0&0&0&0&0 \\ 0&0&0&1&0\\0&0&0&0&0 \end{bmatrix} + 2^{1}\begin{bmatrix}0 & 0 & 0 &0 &0 \\ 0&0 &0 &0&0 \\ 0&0&0&0&0 \\ 0&0&0&0&0\\0&0&0&0&0 \end{bmatrix} + 2^{2}\begin{bmatrix}1 & 0 & 0 &0 &0 \\ 0&0 &0 &0&0 \\ 0&0&0&0&0 \\ 0&0&0&0&0\\0&0&0&0&1 \end{bmatrix} \nonumber\\
    &=2^{-1}\begin{bmatrix}-1 & 0 & 0 &0 &0 \\ 0&1 &0 &0&0 \\ 0&0&-1&0&0 \\ 0&0&0&1&0\\0&0&0&0&-1 \end{bmatrix}+2^{0}\begin{bmatrix}-1 & 0 & 0 &0 &0 \\ 0&-1 &0 &0&0 \\ 0&0&-1&0&0 \\ 0&0&0&-1&0\\0&0&0&0&-1 \end{bmatrix}+2^{1}\begin{bmatrix}1 & 0 & 0 &0 &0 \\ 0&-1 &0 &0&0 \\ 0&0&-1&0&0 \\ 0&0&0&-1&0\\0&0&0&0&1 \end{bmatrix} 
    \nonumber\\
    &+\frac{2^3-1}{2}\begin{bmatrix}1 & 0 & 0 &0 &0 \\ 0&1 &0 &0&0 \\ 0&0&1&0&0 \\ 0&0&0&1&0\\0&0&0&0&1 \end{bmatrix}
\end{align}

\subsection*{Odd summation.}
Here is an alternative to the naive signature sum, which avoids the need to square any integers.

\subsubsection*{Assumptions}
\begin{itemize}
    \item $n$ qubits per link
    \item Electric field states represented by states $\ket{\epsilon}$ of a binary register:
    \begin{align}
        0 \leq  & \epsilon \leq 2^n-1 \\
        E_{\text{min}} \leq & E \leq E_{\text{max}}
        \end{align}
        When it is necessary to consider the binary expansion of $\epsilon$, we write
        \begin{equation}
            \epsilon = \epsilon_{n-1} \epsilon_{n-2} \cdots \epsilon_1 \epsilon_0 = \sum_{k=0}^{n-1} 2^k \epsilon_k
        \end{equation}
    \item The following choice of cutoff and bounds on $E$:
        \begin{align}
        K&=2^{n-1} \\
        E_{\text{min}} &= -K \\
        E_{\text{max}}&=K-1 
        \end{align}
        (The point of taking $-K \leq E \leq K-1$ is that later on we can look at the leading bit of $\epsilon$ to determine whether or not $E(\epsilon)$ is negative.)
        These imply the following conversion between $\epsilon$ and $E$:
        \begin{align}
        E(\epsilon) &= \epsilon + E_{\text{min}} = \epsilon - K \\
        \epsilon(E) &= E - E_{\text{min}} = E + K
    \end{align}
\end{itemize}

\subsubsection*{The sum of unitaries}
\emph{Claim.} Up to an unimportant additive shift (proportional to identity), the electric Hamiltonian $H_E$ is a sum of unitaries taking the following form:
\begin{align}
    \hat{E}^2 &= \sum_{j=0}^{K-1} \alpha_j \hat{U}_j + \text{const.}\\
    \alpha_j &= \frac{1}{2}(2j + 1) \\
    \bra{\epsilon^\prime} \hat{U}_j \ket{\epsilon} &= \delta_{\epsilon^\prime \epsilon} \begin{cases}
    +1 \ , & |E(\epsilon)| > j\\
    -1 \ ,& |E(\epsilon)| \leq j \\
    \end{cases}
\end{align}

This sum is essentially implementing the elementary identity
\begin{equation}
    \sum_{i=0}^{N-1} (2i+1) = N^2
\end{equation}
The coefficients $\alpha_j$ are nothing but the odd numbers in the sum, with an extra factor $1/2$ resulting from using Pavel's trick to turn diagonal matrices with zeroes on the diagonal into signature matrices.

\subsubsection*{Simple example}
Here's the three-qubit version.
Since all the matrices are diagonal it is sufficient to just display the vector of diagonal entries.
\begin{equation}
\begin{split}
    \left( \begin{array}{c}
    16\\9\\4\\1\\0\\1\\4\\9
    \end{array}\right) & = 
    1\left( \begin{array}{c}
    1\\1\\1\\1\\0\\1\\1\\1\\
    \end{array}\right) +
    3\left( \begin{array}{c}
    1\\1\\1\\0\\0\\0\\1\\1\\
    \end{array}\right) +
    5\left( \begin{array}{c}
    1\\1\\0\\0\\0\\0\\0\\1\\
    \end{array}\right) +
    7\left( \begin{array}{c}
    1\\0\\0\\0\\0\\0\\0\\0\\
    \end{array}\right) \\
    & = 
    \frac{1}{2}\left( \begin{array}{c}
    1\\1\\1\\1\\-1\\1\\1\\1\\
    \end{array}\right) +
    \frac{3}{2}\left( \begin{array}{c}
    1\\1\\1\\-1\\-1\\-1\\1\\1\\
    \end{array}\right) +
    \frac{5}{2}\left( \begin{array}{c}
    1\\1\\-1\\-1\\-1\\-1\\-1\\1\\
    \end{array}\right) +
    \frac{7}{2}\left( \begin{array}{c}
    1\\-1\\-1\\-1\\-1\\-1\\-1\\-1\\
    \end{array}\right) + 
    \frac{1+3+5+7}{2} \left( \begin{array}{c}
    1\\1\\1\\1\\1\\1\\1\\1\\
    \end{array}\right)
    \end{split}
\end{equation}

\subsection*{General Method}
\begin{lemma}
Let $E(x) = K - x$ for $x\in \{0,\ldots, 2K-1\}$, then the matrix ${\rm diag}(E(x)^2)\in \mathbb{C}^{2K\times 2K}$ can be implemented as a sum of unitaries of the form $\sum_{j=0}^{K} \alpha_j u_j$ with $$\alpha_j = \begin{cases} \frac{1}{2}(2j+1) & \text{if $j < K$}\\
\frac{K^2}{2} & \text{if $j=K$}
\end{cases}$$ and
$$\bra{x^\prime-K} \hat{U}_j \ket{x-K} = \delta_{x^\prime x} \begin{cases}
    +1 \ , & |x-K| > j\\
    -1 \ ,& |x-K| \leq j \\
    \end{cases}.$$
\end{lemma}
\begin{proof}
The proof follows from direct computation.  By construction each $U_j$ is diagonal, and so we can ignore all off diagonal elements which are trivially zero as desired.
Thus for any $x\in \{K,\ldots, 2K-1\}$
\begin{align}
    \sum_j \alpha_j \bra{x} U_j \ket{x} &= \frac{K^2}{2} + \sum_{j<x-K} \frac{(2j+1)}{2}-\sum_{j\ge x-K} \frac{(2j+1)}{2}\\
    &=\frac{K^2}{2} + 2\sum_{j=0}^{x-K-1} \frac{(2j+1)}{2}-\sum_{j=0}^{K-1} \frac{(2j+1)}{2}\\
    &=(x-K)^2.
\end{align}
Next consider the case where $x\in \{0,\ldots, K-1\}$:
\begin{align}
    \sum_j \alpha_j \bra{x} U_j \ket{x} &= \frac{K^2}{2} + \sum_{j<K-x} \frac{(2j+1)}{2}-\sum_{j\ge K-x} \frac{(2j+1)}{2}\nonumber\\
    &= \frac{K^2}{2} + 2\sum_{j=0}^{K-x-1} \frac{(2j+1)}{2}-\sum_{j=0}^{K-1} \frac{(2j+1)}{2}\\
    &= (K-x)^2.
\end{align}
Therefore our claim holds for all $x$.
\end{proof}
\subsubsection*{How to implement the $U_j$}
The action of $U_j$ on any state $\ket{\epsilon}$ can be summarized as ``phase flip $\ket{\epsilon}$ if and only if $j-|E(\epsilon)|\geq 0$.''
We can proceed by considering the two following possibilities:
\begin{enumerate}
    \item Case $|E(\epsilon)| = E(\epsilon) $. This is equivalent to having the leading bit $\epsilon_{n-1}=1$.\\
    In this case, we have $j-|E(\epsilon)|= j-E(\epsilon) = j+K-\epsilon$.
    Thus, we should compute as follows:
    \begin{equation}
        \ket{j}^n \ket{\epsilon}^n \ \rightarrow \ \ket{j+K}^{n+1} \ket{\epsilon}^n \ \rightarrow \ \ket{j+K - \epsilon}^{n+2} \ket{\epsilon}^n \ ;
    \end{equation}
    then phase flip if and only if $\ket{j+K - \epsilon}$ did not go negative; and finally uncompute the arithmetic.
    \item Case $|E(\epsilon)| \neq E(\epsilon) $. This is equivalent to having the leading bit $\epsilon_{n-1}=0$.\\
    In this case, we have $j-|E(\epsilon)|= j+E(\epsilon) = j+\epsilon-K $.
    Thus, we should compute as follows:
    \begin{equation}
        \ket{j}^n \ket{\epsilon}^n \ \rightarrow \ \ket{j+\epsilon}^{n+1} \ket{\epsilon}^n \ \rightarrow \ \ket{j+\epsilon- K}^{n+2} \ket{\epsilon}^n \ ;
    \end{equation}
    then phase flip if and only if $\ket{j+\epsilon-K}$ did not go negative; and finally uncompute the arithmetic.
\end{enumerate}
The above steps will apply the desired phase to $\ket{\epsilon}$.

For any fixed $U_j$, we see that we can effect its action on an electric field ket using only a constant number of addition and subtraction circuits (without any implicit multiplier circuit), so the gate count scaling will be dominated by the adder algorithm.


